On Higher Dimensional Self-Similar Axion-Dilaton Solutions

We show that solutions of the self-similar gravitational collapse in the Einstein-axion-dilaton system exist in higher dimensional spacetimes. These solutions are invariant under spacetime dilation combined with internal SL(2,R) transformations. We rely on the recent setup and use it for the three different conjugacy classes (elliptic, parabolic and hyperbolic) in higher dimensions. Lastly, we identify new families of physically distinguishable self-similar solutions for all three conjugacy classes in six and seven dimensions.

==> 2005.11646 2 2/6Dhyper/6Dhyper.tex <==
\textcolor{red}{CAREFUL: ALL FIGURES IN THIS SECTION HAVE TO BE UPDATED WITH THE CORRECT LABELS FOR THE SOLUTIONS! The text however should be correct.}

%%%%%%%%%% alpha %%%%%%%%%%
\subsection{Solution branch $\alpha$}

\begin{eqaed}
    w & = 0.00755474 \\
    Im f(0) &= 0.000595673 \\
    z_+ &= 2.70575
\end{eqaed}

quality

\begin{eqaed}
    \text{StoppingObjectiveFunction} &\approx 10^{-10} \\
    b(z)-z-\delta &= 0.-2.00103\times 10^{-7} i \\
\end{eqaed}

\begin{figure}[h!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{6Dhyper/6Dhyper_sol_alpha_PlotPoints40.pdf}
    \caption{Solution branch $\alpha$: contour plot.}
    \label{}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{6Dhyper/6Dhyper_sol_alpha_b2-z2.pdf}
    \caption{Solution branch $\alpha$: $|b^2(z)-z^2|$.}
    \label{}
\end{figure}


\newpage
%%%%%%%%%% beta %%%%%%%%%%
\subsection{Solution branch $\beta$}


\begin{eqaed}
    w & = 0.00225266 \\
    Im f(0) &= 0.000360402 \\
    z_+ &= 1.88269
\end{eqaed}

quality

\begin{eqaed}
    \text{StoppingObjectiveFunction} &\approx 10^{-12} \\
    b(z)-z-\delta &= 0.+1.5836\times 10^{-7} i \\
\end{eqaed}

\begin{figure}[!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{6Dhyper/6Dhyper_sol_gamma_PlotPoints40.pdf}
    \caption{Solution branch $\beta$: contour plot.}
    \label{}
\end{figure}

\begin{figure}[!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{6Dhyper/6Dhyper_sol_gamma_b2-z2.pdf}
    \caption{Solution branch $\beta$: $|b^2(z)-z^2|$.}
    \label{}
\end{figure}

\textcolor{blue}{This one looks really good!}



\newpage
%%%%%%%%%% gamma %%%%%%%%%%
\subsection{Solution branch $\gamma$}

\textcolor{red}{This is the one I found by looking at the 3D plots of SOF.}

\begin{eqaed}
    w & = 0.00105698 \\
    Im f(0) &= 0.00763054 \\
    z_+ &= 1.00079
\end{eqaed}

quality

\begin{eqaed}
    \text{StoppingObjectiveFunction} &\approx 10^{-9} \\
    b(z)-z-\delta &= 2.22045\times 10^{-16}+5.45311\times 10^{-9} i \\
\end{eqaed}

FIGURE TO DO
\begin{figure}[!]
    \centering
    %\includegraphics[width=1\textwidth,keepaspectratio]{6Dhyper/6Dhyper_sol_beta_PlotPoints40.pdf}
    \caption{Solution branch $\gamma$: contour plot.}
    \label{}
\end{figure}

\begin{figure}[!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{6Dhyper/6Dhyper_sol_beta_b2-z2.pdf}
    \caption{Solution branch $\gamma$: $|b^2(z)-z^2|$.}
    \label{}
\end{figure}



\newpage
%%%%%%%%%% delta %%%%%%%%%%
\subsection{Solution branch $\delta$}

\begin{eqaed}
    w & = 0.00020378 \\
    Im f(0) &= 0.0013195 \\
    z_+ &= 1.00101
\end{eqaed}

quality

\begin{eqaed}
    \text{StoppingObjectiveFunction} &\approx 10^{-11} \\
    b(z)-z-\delta &= 2.22045\times 10^{-16}+9.84981\times 10^{-8} i \\
\end{eqaed}

\begin{figure}[!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{6Dhyper/6Dhyper_sol_delta_PlotPoints40.pdf}
    \caption{Solution branch $\gamma$: contour plot.}
    \label{}
\end{figure}

\begin{figure}[!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{6Dhyper/6Dhyper_sol_delta_b2-z2.pdf}
    \caption{Solution branch $\gamma$: $|b^2(z)-z^2|$.}
    \label{}
\end{figure}



\newpage
%%%%%%%%%% a %%%%%%%%%%
\subsection{Non-solution branch $a$}

\textcolor{red}{See Mathematica file please.}

\textcolor{blue}{Looking at the plot, it seems like there should be a solution around $\omega\approx 1.9$. However FindRoot gives error, the error is not low enough and $z_+$ is too large (around $90$) so this seems not to be a solution.}

==> 2005.11646 2 2/6d7dhyper.tex <==

\newpage

\textbf{\textcolor{blue}{GENERAL REMARK ABOUT 6 AND 7 DIMENSIONS HYPERBOLIC CLASS}}\\

 hence we run again the code, lowering some parameters that are introduced for numerical purposes and that are expected to dominate the errors.
%In particular, these parameters are: $z_0=0.001$, the starting point of integration, since we cannot start numerical integration from the singularity $z=0$; and $\delta$.
We checked in lower dimensions, both for elliptic and for hyperbolic class, that the solutions we presented above do not vary if we lower the parameters: hence we believe them to be particularly stable. We cannot claim the same for the hyperbolic class in six and seven dimensions. We were indeed able to find some roots, but they are not as stable as the previous ones. Besides, we cannot recognize them clearly as intersections in the plots of vanishing real and imaginary parts of $G(\omega,\Im f(0))$, due to the noise: for this reason we will not report them here.
All in all, we could not rely on the graphical visualization to get hints as to where the intersections may lie: but the numerical procedure does find some roots with very high precision. 

%%%%%%%%%% 6d hyperbolic %%%%%%%%%%

\subsubsection{Solutions for \texorpdfstring{$d=6$}{d=6} hyperbolic class}

%OLD
%\begin{figure}[h!]
%    \centering
%    \includegraphics[width=3.5in,keepaspectratio]{6Dhyper/6Dhyper_sol_alpha_b2-z2.pdf}
%    \caption{Profile of $\alpha$ solution in 6d hyperbolic case.
%    %Solution branch $\alpha$: $|b^2(z)-z^2|$.
%    }
%    \label{fig:6dsolhyperalpha}
%\end{figure}

%OLD
%\begin{figure}[h!]
%    \centering
%    \includegraphics[width=3.5in,keepaspectratio]{6Dhyper/6Dhyper_sol_all_PlotPoints30_UpdatedLabels.pdf}
%    \caption{Solutions 6d hyperbolic.}
%    \label{fig:6dsolhyper}
%\end{figure}

%We present the first solutions that were found, running the code with the same parameters that have been used for previous classes and dimensions:

%OLD
%\begin{center}
%\bgroup
%\def\arraystretch{2}
%\begin{tabular}{|c|c|c|c|}\hline
   % Solution & $w$ & $\Im f(0)$ & $z_+$ \\ \hline
 %   $\alpha$ & $0.00755474$ & $0.000595673$ & $2.70575$\\
  %  $\beta$ & $0.00225266$ & $0.000360402$ & $1.88269$\\
    %$\gamma$ & $0.00105698$ & $0.00763054$ & $1.00079$\\ zplus is too small with respect to the others!
  %  $\gamma$ & $0.000245789$ & $0.00119848$ & $1.00185$\\
  %  \hline
%\end{tabular}
%\egroup
%\end{center}


Then we run the code again and find the following solutions:

\textcolor{red}{$z_0=0.0001$, $\delta=10^{-5}$, $overlap=0.1$}

%OLD TABLE
%\begin{center}
%\bgroup
%\def\arraystretch{2}
%\begin{tabular}{|c|c|c|c|}\hline
%    Solution & $w$ & $\Im f(0)$ & $z_+$ \\ \hline
%    $\alpha$ & $0.0109996$ & $0.00100003$ & $2.5169$\\
%    $\beta$ & $0.00789925$ & $0.000601004$ & $2.75526$\\
%    $\gamma$ & $0.00170467$ & $0.00094809$ & $1.13803$\\
%    $\delta$ & $0.00114537$ & $0.00197762$ & $1.01546$\\
%    $\epsilon$ & $0.000171151$ & $0.000224557$ & $1.02661$\\
%    \hline
%\end{tabular}
%\egroup
%\end{center}

%NEWEST TABLE (the numbers are those of the handwritten page!)

\begin{center}
\bgroup
\def\arraystretch{2}
\begin{tabular}{|c|c|c|c|c|}\hline
    Solution & $w$ & $\Im f(0)$ & $z_+$ & Error \\ \hline
    $\alpha$ & $0.0100$ & $0.0070$ & $1.0901$ & $10^{-10}$\\
    $\beta$ & $0.0063$ & $0.0038$ & $1.1201$ & $10^{-11}$\\
    %with all digits:
    %$(4)$ & $0.010009$ & $0.007003$ & $1.09005$ & $10^{-10}$\\
    %$(7)$ & $0.00629968$ & $0.00377983$ & $1.12005$ & $10^{-11}$\\
    %$(1)$ & $0.00430836$ & $0.00689293$ & $1.01798$ & $10^{-10}$\\
    %$(10)$ & $0.0036901$ & $0.00170595$ & $1.19228$ & $10^{-11}$\\
    %$(5)$ & $0.00118053$ & $0.00191215$ & $1.01755$ & $10^{-12}$\\
    \hline
\end{tabular}
\egroup
\end{center}



%In Figure \ref{fig:6dsolhyper} the profile of the $\alpha$ solution is shown \textcolor{red}{to be drawn again for the correct $\alpha$ since I want to rule out the current one...}

%\begin{figure}[h!]
   % \centering
 %   \includegraphics[width=3.5in,keepaspectratio]{6Dhyper_sol_alpha_PlotPoints20_1.pdf}
  %  \caption{The curves of vanishing real and imaginary parts of the constraint around the $\alpha$ solution in the six dimensional hyperbolic case. \textcolor{red}{Do we keep this one?}}
 %   \label{fig:6dsolhyperalpha}
%\end{figure}

%\begin{figure}[h!]
 %   \centering
  %  \includegraphics[width=2.5in,keepaspectratio]{6Dhyper_sol_alpha_b2-z2.pdf}
   % \caption{The profile for the $\alpha$ solution in the six dimensional hyperbolic case.}
    %|b2-z2|
  %  \label{fig:6dsolhyper}
%\end{figure}

\textcolor{blue}{In general, for the hyperbolic class in five, six and seven dimensions we could find and underlying common behavior for the solutions. We notice that, as $\omega$ decreases, the singularity $z_+$ also decreases.}

\textcolor{red}{ We highlight that, as it is to be expected, the numerical procedure is more and more affected by noise as the dimension of space-time increases. We might maybe mention that we tried to use these plots as hints to where a solution might lie, but the constraint is very noisy and this procedure is difficult. 

If we decide to show some plots of the vanishing real and imaginary parts we might as well add a contour plot of the constraint, in order to show the noise and the fact that we cannot spot any intersection from a graphical point of view. FOR THESE HIGH DIMENSIONS WE COULD ONLY RELY ON THE NUMERICAL ROOTFINDING PROCEDURE.}



\newpage

%%%%%%%%%% 7d hyperbolic %%%%%%%%%%

\subsubsection{Solutions for \texorpdfstring{$d=7$}{d=7}, hyperbolic class}

\textcolor{red}{$z_0=0.0001$, $\delta=10^{-5}$, $overlap=0.1$}

\begin{center}
\bgroup
\def\arraystretch{2}
\begin{tabular}{|c|c|c|c|c|}\hline
    Solution & $w$ & $\Im f(0)$ & $z_+$ & Error \\ \hline
    $\alpha$ & $0.0021$ & $0.0014$ & $1.0828$ & $10^{-12}$\\
    $\beta$ & $0.0017$ & $0.0011$ & $1.0952$ & $10^{-11}$\\
    %$\delta$ & $0.0011$ & $0.0020$ & $1.0155$\\
    %all digits
    %$\alpha$ & $0.00211549$ & $0.00143006$ & $1.0828$\\
    % $\beta$ & $0.001699$ & $0.001067$ & $1.09516$ & $10^{-11}$\\
    %$\delta$ & $0.00114537$ & $0.00197762$ & $1.01546$\\
    %$\epsilon$ & $0.000171151$ & $0.000224557$ & $1.02661$\\
    \hline
\end{tabular}
\egroup
\end{center}

%


%%% %%% %%%
 We highlight that, as it is to be expected, the numerical procedure is more and more affected by noise as the dimension of space-time increases. We might maybe mention that we tried to use these plots as hints to where a solution might lie, but the constraint is very noisy and this procedure is difficult. 

If we decide to show some plots of the vanishing real and imaginary parts we might as well add a contour plot of the constraint, in order to show the noise and the fact that we cannot spot any intersection from a graphical point of view. FOR THESE HIGH DIMENSIONS WE COULD ONLY RELY ON THE NUMERICAL ROOTFINDING PROCEDURE.
\section{News about 6d hyperbolic}
I ran the code with $z_0=0.0001$, $\text{overlap}=0.1$, $\delta=10^{-5}$ and compared to our old parameters $z_0=0.001$, $\text{overlap}=0.1$, $\delta=10^{-4}$.
\begin{itemize}
    \item First of all, lowering the parameters I get many more solutions than I used to, comparing the very same regions with the same starting guesses.
    \item Solutions are found randomly far away from the starting guesses. There seems to be no link at all between the starting guesses I plug in and the results of FindRoot (but this is general to six and seven dimensions, we've already seen it many times).
    \item Solutions seem to have a weird tendency to cluster around integer values of $\omega$. I will show you the plot.
    \item There seem to be a link among the magnitude of $z_+$ and the shape of the plot $b^2-z^2$. Solutions can be classified according to these criteria, see the following figure: values of $z_+$ close to $1$ have a nice shape $\alpha$, while values greater than more or less $2$ have shape $\beta$.
    \item If I consider all the $\alpha$ solutions alone, they do not respect our trend (decreasing $\omega$ - decreasing $z_+$). Similarly, the $\beta$ solutions alone do not respect the trend. There's no clear reason to discard points.
\end{itemize}
\begin{figure}[h!]
\centering
\begin{subfigure}[t]{.5\textwidth}
  \centering
  \includegraphics[width=.99\linewidth]{6Dhyper_b2-z2_shapeALFA.pdf}
  \caption{Shape $\alpha$.}
  \label{}
\end{subfigure}%
\begin{subfigure}[t]{.5\textwidth}
  \centering
  \includegraphics[width=.99\linewidth]{6Dhyper_b2-z2_shapeBETA.pdf}
  \caption{Shape $\beta$.}
  \label{}
\end{subfigure}
\caption{Shapes of $b^2-z^2$.}
\label{}
\end{figure}






%\section{d=6 hyperbolic}
%\import{}{6Dhyper/6Dhyper.tex}

%\section{d=7 hyperbolic}
%\import{}{7Dhyper/7Dhyper.tex}

==> 2005.11646 2 2/7Dhyper/7Dhyper.tex <==
%\textcolor{red}{1.  THE SAME DELTA =.0001 }

 
%\textcolor{red}{ from minus part up to zero for Imf(0), with z+=.001 and overlap.1 and delta .0001}

 




%%%%%%%%%% alpha %%%%%%%%%%
\subsection{Solution branch $\alpha$}

\begin{eqaed}
    w & = 0.00491925 \\
    Im f(0) &= 0.00219029 \\
    z_+ &= 1.17835
\end{eqaed}

quality\\
\textcolor{red}{FindRoot gives error}

\begin{eqaed}
    \text{StoppingObjectiveFunction} &\approx 10^{-10} \\
    b(z)-z-\delta &= 0.+3.78798\times 10^{-7} i \\
\end{eqaed}

\begin{figure}[!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{7Dhyper/7Dhyper_sol_alpha_zoomed_PlotPoints40.pdf}
    \caption{Solution branch $\alpha$: contour plot.}
    \label{}
\end{figure}





%%%%%%%%%% beta %%%%%%%%%%
\subsection{Solution branch $\beta$}



\begin{eqaed}
    w & = 0.01155 \\
    Im f(0) &= 0.00171688 \\
    z_+ &= 1.8646
\end{eqaed}

quality\\
\textcolor{red}{FindRoot gives error}

\begin{eqaed}
    \text{StoppingObjectiveFunction} &\approx 10^{-10,9} \\
    b(z)-z-\delta &= 0.+1.47933\times 10^{-8} i \\
\end{eqaed}

\begin{figure}[!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{7Dhyper/7Dhyper_sol_beta_zoomed_PlotPoints40.pdf}
    \includegraphics[width=1\textwidth,keepaspectratio]{7Dhyper/7Dhyper_sol_beta_zoomedIN_PlotPoints40.pdf}
    \caption{Solution branch $\beta$: contour plot.}
    \label{}
\end{figure}

\begin{figure}[!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{7Dhyper/7Dhyper_sol_beta_b2-z2.pdf}
    \caption{Solution branch $\beta$: $|b^2(z)-z^2|$.}
    \label{}
\end{figure}



%%%%%%%%%% beta %%%%%%%%%%
%\subsection{Solution branch $\gamma$}

%\begin{eqaed}
 %   w & = 2.21223 \\
   % Im f(0) &= 0.000462928 \\
 %   z_+ &= 65.2425
%\end{eqaed}


%\begin{figure}[!]
  %  \centering
  %  \includegraphics[width=1\textwidth,keepaspectratio]{7Dhyper/7Dhyper_sol_beta_zoomed_PlotPoints40.pdf}
  %  \includegraphics[width=1\textwidth,keepaspectratio]{7Dhyper/7Dhyper_sol_gamma_PlotPoints40.pdf}
  %  \caption{Solution branch $\beta$: contour plot.}
   % \label{}
%\end{figure}



%\textcolor{green}{The error is comparable with $Im(f)0))$, besides $z_+$ is very large. it isnot a solution.}

==> 2005.11646 2 2/notes_from_papers.tex <==
\section{Universality and Scaling in Gravitational Collapse of a Massless Scalar Field\\M. W. Choptuik}

Problem: single massless scalar field $\phi$ minimally coupled to gravity $g_{\mu\nu}$.

It is an arena to investigate the nature and consequence of nonlinearity in General Relativity.

The general time-dependent, spherically symmetric metric is:
\begin{equation}
    ds^2=-\alpha^2(r,t)dt^2+a^2(r,t)dr^2+r^2d\Omega^2
\end{equation}
The system of equations obtained for the field and for the functions $\alpha$ and $a$ is \textbf{invariant under rescalings}
\begin{align}
    &r\xrightarrow{}kr\\
    &t\xrightarrow{}kt\\
    &k>0
\end{align}
This amounts to a choice of units, and reflects the \textbf{absence of a mass/length scale in the model}.

Choptuik studies one-parameter families of solutions $\mathcal{S}[p]$. The parameter $p$ characterizes the strength of the gravitational self-interaction of the scalar field. These solutions are obtained by evolving initially in-going packets (shells) of scalar field.\\
For each family there is a value $p_{weak}$ such that in the limit $p\xrightarrow{}p_{weak}$ you recover flat spacetime and the scalar field evolution is simply a solution of the linear wave equation: the scalar wavepacket implodes through $r=0$ and then escapes to infinity (\textcolor{red}{?}).\\
At the other extreme, there is a value $p_{strong}$ such that in the limit $p\xrightarrow{}p_{strong}$ you end up forming a black hole in the collapse of the packet, and an arbitrarily small fraction of the scalar field escapes to infinity (\textcolor{red}{does it mean that we would need to wait an infinite time to see that fraction at infinity? Or is it just the asymptotic behaviour, so that in the exact $p_{strong}$ case you would see nothing at infinity?}).\\
In between there is, geometrically, a \textbf{critical parameter} value $p^*$ where black hole formation first occurs. We can assume $p_{weak}<p^*<p_{strong}$ and refer to solutions as subcritical and supercritical according to whether we are below or above $p^*$. The quantity $|p-p^*|$ is, in both regimes, a natural choice to discuss the phenomenology of the solutions.

In the strong-field, near-critical dynamics $p\xrightarrow{}p^*$ Choptuik conjectures that:\\
(1) the precisely critical behaviour is universal (independent of the particular initial profile chosen for the field);\\
(2) in terms of certain variables, the field profiles of the critical evolution at frozen time will be the same as one rescales the variables by some universal constant $\Delta$. In other words, if one looks at the profiles at a certain geometric time $T$ and then at a later time on scales $e^{\Delta}$ smaller, then the same profiles will appear; then one waits for an additional interval $\delta T$ and zooms in by an additional factor $e^{\Delta}$, again the same profiles.\\
This only happens for strong-field dynamics, that is we are close to $r=0$.

\textbf{A precisely critical configuration will be characterized by an infinite series of echoes in the field profiles, as well as in any other form-invariant quantity} such as $a$, $m/r$, $dm/dr$... which arise from dynamics unfolding on increasingly smaller spatiotemporal scales. There is a geometric relation between the scales of successive echoes: the sequence will conclude at some \textbf{finite} central proper time $T^*$.

One can study the critical behavior starting from subcritical solutions or also from supercritical. In the latter case, \textbf{empirically, the black hole mass is well described by a powerlaw}
\begin{equation}
    M_{BH}\approx c_f |p-p^*|^{\gamma}
\end{equation}
where $c_f$ is a constant that depends on the family, but $\gamma$ is apparently universal and has a numerical value $\gamma\approx 0.37$.



\section{Universal Scaling and Echoing in Gravitational Collapse of a
Complex Scalar Field\\E. W. Hirschmann and D. M. Eardley}

\textbf{Gravitational collapse has two kinds of possible endstates}. The ﬁrst endstate consists of a \textbf{black hole}, plus some outgoing matter and outgoing gravitational radiation. The second endstate consists of a \textbf{stationary remnant star}, plus some outgoing matter and outgoing gravitational radiation, but no black hole. Choice between these endstates \textbf{depends on initial conditions}; gravitational collapse ends in a black hole only if the gravitational ﬁeld becomes strong enough, in the sense of the singularity theorems. A third possibility, the \textbf{naked} singularity, is thought not to occur due to the cosmic censorship conjecture.

The thought experiment employed by Choptuik, in the context of numerical relativity, is to \textbf{tune across the critical threshold in the space of initial conditions} and study the behavior of quantities at this threshold. The parameter $p$ he chose describes the stregth of gravity in the initial state. He finds evidence that the threshold behavior is somehow universal...

For gravitational collapse of \textbf{fermionic matter} from suitably regular initial conditions, the Chandrasekhar mass sets the scale of minimum mass for any black hole, as long as the initial conditions are suﬃciently regular (meaning we don't use focused beams of ultrarelativistic fermions or something like that). In this case, the black hole mass $M_{BH}(p)$ for fermionic configurations  behaves in a simple and rather uninteresting way at threshold: \textbf{it is a step function of} $p$.

For gravitational collapse of \textbf{bosonic matter} from regular initial conditions, we do not find a step function! In spherically symmetric collapse of a massless real scalar ﬁeld $\phi$ coupled to gravity, Choptuik ﬁnds a \textbf{power-law behavior}
\begin{equation}
    M_{BH}(p) \approx (p-p^*)^{\gamma} \qquad \gamma \approx 0.37
\end{equation}
and conjectures that $\gamma$ may be universal.


 For a massless scalar ﬁeld with no self-coupling, no bound star can exist (\textcolor{red}{is that because there is nothing that may play the role of pressure?} so that we either collapse due to gravity or blow away at infinity?), so that the endstate consists of outgoing scalar radiation, plus a possible black hole.
 
 Furthermore, exactly at the threshold
  $ p^* $
 
 , he ﬁnds a unique ﬁeld conﬁguration acting as an attractor for all nearby initial conditions. This ﬁeld conﬁguration, which we will call a \textbf{choptuon}, has a \textbf{discrete self-similarity}, by virtue of which it exhibits a striking, recurrent \textbf{echoing behavior: it repeats itself at ever-decreasing time- and length-scales}.
 \begin{align}
     &\phi(t^{\prime},r^{\prime})=\phi(t,r)\\
     &t^{\prime}=e^{-n\Delta}t \qquad r^{\prime}=e^{-n\Delta}r \qquad ds^{\prime 2}=e^{-2n\Delta}ds^2 \qquad n=1,2,3,...
 \end{align}
 with $(t,r)$ spherical coordinates and $\Delta$ a constant to be determined numerically. The solution is thus \textbf{invariant under a discrete family of scale transformations}.
 
 \textcolor{red}{Choptuons amount to a new kind of counterexample to some formulations of the cosmic censorship conjecture}, a counterexample that cannot be blamed on bad choice of matter ﬁelds. Technically they are a counterexample because regions of arbitrarily strong curvature are visible to observers at future null inﬁnity.\\
 Even more importantly, choptuons represent in principle a means by which eﬀects of extremely strong ﬁeld gravity, even quantum gravity, can be observable in the present universe.
 
 If we use a \textbf{complex scalar field} rather than a real one, echoing is allowed to occur in the form of \textbf{phase oscillations}: $\phi$ changes phase but not amplitude under a scale transformation. In other words, we can interpret the rescaling as acting on the amplitude, or on the phase, or both.
 \begin{align}
     &\phi(t,r)=(-t)^{i\omega}f(-r/t)\\
     &t^{\prime}=e^{-\lambda}t \qquad r^{\prime}=e^{-\lambda}r \qquad \phi(t^{\prime},r^{\prime})=e^{-i\omega\lambda}\phi(t,r) \qquad 0<\lambda<\infty
 \end{align}
 This field is continuously self-similar. It exhibits \textbf{linear phase oscillations, a form of the echoing, superimposed on exact continuous scale symmetry}.



\section{More On Critical Collapse of Axion-Dilaton System in Dimension Four
\\L. \'Alvarez-Gaumé and Ehsan Hatefi}

==> 6Dhyper/6Dhyper.tex <==
\textcolor{red}{CAREFUL: ALL FIGURES IN THIS SECTION HAVE TO BE UPDATED WITH THE CORRECT LABELS FOR THE SOLUTIONS! The text however should be correct.}

%%%%%%%%%% alpha %%%%%%%%%%
\subsection{Solution branch $\alpha$}

\begin{eqaed}
    w & = 0.00755474 \\
    Im f(0) &= 0.000595673 \\
    z_+ &= 2.70575
\end{eqaed}

quality

\begin{eqaed}
    \text{StoppingObjectiveFunction} &\approx 10^{-10} \\
    b(z)-z-\delta &= 0.-2.00103\times 10^{-7} i \\
\end{eqaed}

\begin{figure}[h!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{6Dhyper/6Dhyper_sol_alpha_PlotPoints40.pdf}
    \caption{Solution branch $\alpha$: contour plot.}
    \label{}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{6Dhyper/6Dhyper_sol_alpha_b2-z2.pdf}
    \caption{Solution branch $\alpha$: $|b^2(z)-z^2|$.}
    \label{}
\end{figure}


\newpage
%%%%%%%%%% beta %%%%%%%%%%
\subsection{Solution branch $\beta$}


\begin{eqaed}
    w & = 0.00225266 \\
    Im f(0) &= 0.000360402 \\
    z_+ &= 1.88269
\end{eqaed}

quality

\begin{eqaed}
    \text{StoppingObjectiveFunction} &\approx 10^{-12} \\
    b(z)-z-\delta &= 0.+1.5836\times 10^{-7} i \\
\end{eqaed}

\begin{figure}[!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{6Dhyper/6Dhyper_sol_gamma_PlotPoints40.pdf}
    \caption{Solution branch $\beta$: contour plot.}
    \label{}
\end{figure}

\begin{figure}[!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{6Dhyper/6Dhyper_sol_gamma_b2-z2.pdf}
    \caption{Solution branch $\beta$: $|b^2(z)-z^2|$.}
    \label{}
\end{figure}

\textcolor{blue}{This one looks really good!}



\newpage
%%%%%%%%%% gamma %%%%%%%%%%
\subsection{Solution branch $\gamma$}

\textcolor{red}{This is the one I found by looking at the 3D plots of SOF.}

\begin{eqaed}
    w & = 0.00105698 \\
    Im f(0) &= 0.00763054 \\
    z_+ &= 1.00079
\end{eqaed}

quality

\begin{eqaed}
    \text{StoppingObjectiveFunction} &\approx 10^{-9} \\
    b(z)-z-\delta &= 2.22045\times 10^{-16}+5.45311\times 10^{-9} i \\
\end{eqaed}

FIGURE TO DO
\begin{figure}[!]
    \centering
    %\includegraphics[width=1\textwidth,keepaspectratio]{6Dhyper/6Dhyper_sol_beta_PlotPoints40.pdf}
    \caption{Solution branch $\gamma$: contour plot.}
    \label{}
\end{figure}

\begin{figure}[!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{6Dhyper/6Dhyper_sol_beta_b2-z2.pdf}
    \caption{Solution branch $\gamma$: $|b^2(z)-z^2|$.}
    \label{}
\end{figure}



\newpage
%%%%%%%%%% delta %%%%%%%%%%
\subsection{Solution branch $\delta$}

\begin{eqaed}
    w & = 0.00020378 \\
    Im f(0) &= 0.0013195 \\
    z_+ &= 1.00101
\end{eqaed}

quality

\begin{eqaed}
    \text{StoppingObjectiveFunction} &\approx 10^{-11} \\
    b(z)-z-\delta &= 2.22045\times 10^{-16}+9.84981\times 10^{-8} i \\
\end{eqaed}

\begin{figure}[!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{6Dhyper/6Dhyper_sol_delta_PlotPoints40.pdf}
    \caption{Solution branch $\gamma$: contour plot.}
    \label{}
\end{figure}

\begin{figure}[!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{6Dhyper/6Dhyper_sol_delta_b2-z2.pdf}
    \caption{Solution branch $\gamma$: $|b^2(z)-z^2|$.}
    \label{}
\end{figure}



\newpage
%%%%%%%%%% a %%%%%%%%%%
\subsection{Non-solution branch $a$}

\textcolor{red}{See Mathematica file please.}

\textcolor{blue}{Looking at the plot, it seems like there should be a solution around $\omega\approx 1.9$. However FindRoot gives error, the error is not low enough and $z_+$ is too large (around $90$) so this seems not to be a solution.}

==> 6d7dhyper.tex <==

\newpage

\textbf{\textcolor{blue}{GENERAL REMARK ABOUT 6 AND 7 DIMENSIONS HYPERBOLIC CLASS}}\\

 hence we run again the code, lowering some parameters that are introduced for numerical purposes and that are expected to dominate the errors.
%In particular, these parameters are: $z_0=0.001$, the starting point of integration, since we cannot start numerical integration from the singularity $z=0$; and $\delta$.
We checked in lower dimensions, both for elliptic and for hyperbolic class, that the solutions we presented above do not vary if we lower the parameters: hence we believe them to be particularly stable. We cannot claim the same for the hyperbolic class in six and seven dimensions. We were indeed able to find some roots, but they are not as stable as the previous ones. Besides, we cannot recognize them clearly as intersections in the plots of vanishing real and imaginary parts of $G(\omega,\Im f(0))$, due to the noise: for this reason we will not report them here.
All in all, we could not rely on the graphical visualization to get hints as to where the intersections may lie: but the numerical procedure does find some roots with very high precision. 

%%%%%%%%%% 6d hyperbolic %%%%%%%%%%

\subsubsection{Solutions for \texorpdfstring{$d=6$}{d=6} hyperbolic class}

%OLD
%\begin{figure}[h!]
%    \centering
%    \includegraphics[width=3.5in,keepaspectratio]{6Dhyper/6Dhyper_sol_alpha_b2-z2.pdf}
%    \caption{Profile of $\alpha$ solution in 6d hyperbolic case.
%    %Solution branch $\alpha$: $|b^2(z)-z^2|$.
%    }
%    \label{fig:6dsolhyperalpha}
%\end{figure}

%OLD
%\begin{figure}[h!]
%    \centering
%    \includegraphics[width=3.5in,keepaspectratio]{6Dhyper/6Dhyper_sol_all_PlotPoints30_UpdatedLabels.pdf}
%    \caption{Solutions 6d hyperbolic.}
%    \label{fig:6dsolhyper}
%\end{figure}

%We present the first solutions that were found, running the code with the same parameters that have been used for previous classes and dimensions:

%OLD
%\begin{center}
%\bgroup
%\def\arraystretch{2}
%\begin{tabular}{|c|c|c|c|}\hline
   % Solution & $w$ & $\Im f(0)$ & $z_+$ \\ \hline
 %   $\alpha$ & $0.00755474$ & $0.000595673$ & $2.70575$\\
  %  $\beta$ & $0.00225266$ & $0.000360402$ & $1.88269$\\
    %$\gamma$ & $0.00105698$ & $0.00763054$ & $1.00079$\\ zplus is too small with respect to the others!
  %  $\gamma$ & $0.000245789$ & $0.00119848$ & $1.00185$\\
  %  \hline
%\end{tabular}
%\egroup
%\end{center}


Then we run the code again and find the following solutions:

\textcolor{red}{$z_0=0.0001$, $\delta=10^{-5}$, $overlap=0.1$}

%OLD TABLE
%\begin{center}
%\bgroup
%\def\arraystretch{2}
%\begin{tabular}{|c|c|c|c|}\hline
%    Solution & $w$ & $\Im f(0)$ & $z_+$ \\ \hline
%    $\alpha$ & $0.0109996$ & $0.00100003$ & $2.5169$\\
%    $\beta$ & $0.00789925$ & $0.000601004$ & $2.75526$\\
%    $\gamma$ & $0.00170467$ & $0.00094809$ & $1.13803$\\
%    $\delta$ & $0.00114537$ & $0.00197762$ & $1.01546$\\
%    $\epsilon$ & $0.000171151$ & $0.000224557$ & $1.02661$\\
%    \hline
%\end{tabular}
%\egroup
%\end{center}

%NEWEST TABLE (the numbers are those of the handwritten page!)

\begin{center}
\bgroup
\def\arraystretch{2}
\begin{tabular}{|c|c|c|c|c|}\hline
    Solution & $w$ & $\Im f(0)$ & $z_+$ & Error \\ \hline
    $\alpha$ & $0.0100$ & $0.0070$ & $1.0901$ & $10^{-10}$\\
    $\beta$ & $0.0063$ & $0.0038$ & $1.1201$ & $10^{-11}$\\
    %with all digits:
    %$(4)$ & $0.010009$ & $0.007003$ & $1.09005$ & $10^{-10}$\\
    %$(7)$ & $0.00629968$ & $0.00377983$ & $1.12005$ & $10^{-11}$\\
    %$(1)$ & $0.00430836$ & $0.00689293$ & $1.01798$ & $10^{-10}$\\
    %$(10)$ & $0.0036901$ & $0.00170595$ & $1.19228$ & $10^{-11}$\\
    %$(5)$ & $0.00118053$ & $0.00191215$ & $1.01755$ & $10^{-12}$\\
    \hline
\end{tabular}
\egroup
\end{center}



%In Figure \ref{fig:6dsolhyper} the profile of the $\alpha$ solution is shown \textcolor{red}{to be drawn again for the correct $\alpha$ since I want to rule out the current one...}

%\begin{figure}[h!]
   % \centering
 %   \includegraphics[width=3.5in,keepaspectratio]{6Dhyper_sol_alpha_PlotPoints20_1.pdf}
  %  \caption{The curves of vanishing real and imaginary parts of the constraint around the $\alpha$ solution in the six dimensional hyperbolic case. \textcolor{red}{Do we keep this one?}}
 %   \label{fig:6dsolhyperalpha}
%\end{figure}

%\begin{figure}[h!]
 %   \centering
  %  \includegraphics[width=2.5in,keepaspectratio]{6Dhyper_sol_alpha_b2-z2.pdf}
   % \caption{The profile for the $\alpha$ solution in the six dimensional hyperbolic case.}
    %|b2-z2|
  %  \label{fig:6dsolhyper}
%\end{figure}

\textcolor{blue}{In general, for the hyperbolic class in five, six and seven dimensions we could find and underlying common behavior for the solutions. We notice that, as $\omega$ decreases, the singularity $z_+$ also decreases.}

\textcolor{red}{ We highlight that, as it is to be expected, the numerical procedure is more and more affected by noise as the dimension of space-time increases. We might maybe mention that we tried to use these plots as hints to where a solution might lie, but the constraint is very noisy and this procedure is difficult. 

If we decide to show some plots of the vanishing real and imaginary parts we might as well add a contour plot of the constraint, in order to show the noise and the fact that we cannot spot any intersection from a graphical point of view. FOR THESE HIGH DIMENSIONS WE COULD ONLY RELY ON THE NUMERICAL ROOTFINDING PROCEDURE.}



\newpage

%%%%%%%%%% 7d hyperbolic %%%%%%%%%%

\subsubsection{Solutions for \texorpdfstring{$d=7$}{d=7}, hyperbolic class}

\textcolor{red}{$z_0=0.0001$, $\delta=10^{-5}$, $overlap=0.1$}

\begin{center}
\bgroup
\def\arraystretch{2}
\begin{tabular}{|c|c|c|c|c|}\hline
    Solution & $w$ & $\Im f(0)$ & $z_+$ & Error \\ \hline
    $\alpha$ & $0.0021$ & $0.0014$ & $1.0828$ & $10^{-12}$\\
    $\beta$ & $0.0017$ & $0.0011$ & $1.0952$ & $10^{-11}$\\
    %$\delta$ & $0.0011$ & $0.0020$ & $1.0155$\\
    %all digits
    %$\alpha$ & $0.00211549$ & $0.00143006$ & $1.0828$\\
    % $\beta$ & $0.001699$ & $0.001067$ & $1.09516$ & $10^{-11}$\\
    %$\delta$ & $0.00114537$ & $0.00197762$ & $1.01546$\\
    %$\epsilon$ & $0.000171151$ & $0.000224557$ & $1.02661$\\
    \hline
\end{tabular}
\egroup
\end{center}

%


%%% %%% %%%
 We highlight that, as it is to be expected, the numerical procedure is more and more affected by noise as the dimension of space-time increases. We might maybe mention that we tried to use these plots as hints to where a solution might lie, but the constraint is very noisy and this procedure is difficult. 

If we decide to show some plots of the vanishing real and imaginary parts we might as well add a contour plot of the constraint, in order to show the noise and the fact that we cannot spot any intersection from a graphical point of view. FOR THESE HIGH DIMENSIONS WE COULD ONLY RELY ON THE NUMERICAL ROOTFINDING PROCEDURE.
\section{News about 6d hyperbolic}
I ran the code with $z_0=0.0001$, $\text{overlap}=0.1$, $\delta=10^{-5}$ and compared to our old parameters $z_0=0.001$, $\text{overlap}=0.1$, $\delta=10^{-4}$.
\begin{itemize}
    \item First of all, lowering the parameters I get many more solutions than I used to, comparing the very same regions with the same starting guesses.
    \item Solutions are found randomly far away from the starting guesses. There seems to be no link at all between the starting guesses I plug in and the results of FindRoot (but this is general to six and seven dimensions, we've already seen it many times).
    \item Solutions seem to have a weird tendency to cluster around integer values of $\omega$. I will show you the plot.
    \item There seem to be a link among the magnitude of $z_+$ and the shape of the plot $b^2-z^2$. Solutions can be classified according to these criteria, see the following figure: values of $z_+$ close to $1$ have a nice shape $\alpha$, while values greater than more or less $2$ have shape $\beta$.
    \item If I consider all the $\alpha$ solutions alone, they do not respect our trend (decreasing $\omega$ - decreasing $z_+$). Similarly, the $\beta$ solutions alone do not respect the trend. There's no clear reason to discard points.
\end{itemize}
\begin{figure}[h!]
\centering
\begin{subfigure}[t]{.5\textwidth}
  \centering
  \includegraphics[width=.99\linewidth]{6Dhyper_b2-z2_shapeALFA.pdf}
  \caption{Shape $\alpha$.}
  \label{}
\end{subfigure}%
\begin{subfigure}[t]{.5\textwidth}
  \centering
  \includegraphics[width=.99\linewidth]{6Dhyper_b2-z2_shapeBETA.pdf}
  \caption{Shape $\beta$.}
  \label{}
\end{subfigure}
\caption{Shapes of $b^2-z^2$.}
\label{}
\end{figure}






%\section{d=6 hyperbolic}
%\import{}{6Dhyper/6Dhyper.tex}

%\section{d=7 hyperbolic}
%\import{}{7Dhyper/7Dhyper.tex}

==> 7Dhyper/7Dhyper.tex <==
%\textcolor{red}{1.  THE SAME DELTA =.0001 }

 
%\textcolor{red}{ from minus part up to zero for Imf(0), with z+=.001 and overlap.1 and delta .0001}

 




%%%%%%%%%% alpha %%%%%%%%%%
\subsection{Solution branch $\alpha$}

\begin{eqaed}
    w & = 0.00491925 \\
    Im f(0) &= 0.00219029 \\
    z_+ &= 1.17835
\end{eqaed}

quality\\
\textcolor{red}{FindRoot gives error}

\begin{eqaed}
    \text{StoppingObjectiveFunction} &\approx 10^{-10} \\
    b(z)-z-\delta &= 0.+3.78798\times 10^{-7} i \\
\end{eqaed}

\begin{figure}[!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{7Dhyper/7Dhyper_sol_alpha_zoomed_PlotPoints40.pdf}
    \caption{Solution branch $\alpha$: contour plot.}
    \label{}
\end{figure}





%%%%%%%%%% beta %%%%%%%%%%
\subsection{Solution branch $\beta$}



\begin{eqaed}
    w & = 0.01155 \\
    Im f(0) &= 0.00171688 \\
    z_+ &= 1.8646
\end{eqaed}

quality\\
\textcolor{red}{FindRoot gives error}

\begin{eqaed}
    \text{StoppingObjectiveFunction} &\approx 10^{-10,9} \\
    b(z)-z-\delta &= 0.+1.47933\times 10^{-8} i \\
\end{eqaed}

\begin{figure}[!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{7Dhyper/7Dhyper_sol_beta_zoomed_PlotPoints40.pdf}
    \includegraphics[width=1\textwidth,keepaspectratio]{7Dhyper/7Dhyper_sol_beta_zoomedIN_PlotPoints40.pdf}
    \caption{Solution branch $\beta$: contour plot.}
    \label{}
\end{figure}

\begin{figure}[!]
    \centering
    \includegraphics[width=1\textwidth,keepaspectratio]{7Dhyper/7Dhyper_sol_beta_b2-z2.pdf}
    \caption{Solution branch $\beta$: $|b^2(z)-z^2|$.}
    \label{}
\end{figure}



%%%%%%%%%% beta %%%%%%%%%%
%\subsection{Solution branch $\gamma$}

%\begin{eqaed}
 %   w & = 2.21223 \\
   % Im f(0) &= 0.000462928 \\
 %   z_+ &= 65.2425
%\end{eqaed}


%\begin{figure}[!]
  %  \centering
  %  \includegraphics[width=1\textwidth,keepaspectratio]{7Dhyper/7Dhyper_sol_beta_zoomed_PlotPoints40.pdf}
  %  \includegraphics[width=1\textwidth,keepaspectratio]{7Dhyper/7Dhyper_sol_gamma_PlotPoints40.pdf}
  %  \caption{Solution branch $\beta$: contour plot.}
   % \label{}
%\end{figure}



%\textcolor{green}{The error is comparable with $Im(f)0))$, besides $z_+$ is very large. it isnot a solution.}

==> notes_from_papers.tex <==
\section{Universality and Scaling in Gravitational Collapse of a Massless Scalar Field\\M. W. Choptuik}

Problem: single massless scalar field $\phi$ minimally coupled to gravity $g_{\mu\nu}$.

It is an arena to investigate the nature and consequence of nonlinearity in General Relativity.

The general time-dependent, spherically symmetric metric is:
\begin{equation}
    ds^2=-\alpha^2(r,t)dt^2+a^2(r,t)dr^2+r^2d\Omega^2
\end{equation}
The system of equations obtained for the field and for the functions $\alpha$ and $a$ is \textbf{invariant under rescalings}
\begin{align}
    &r\xrightarrow{}kr\\
    &t\xrightarrow{}kt\\
    &k>0
\end{align}
This amounts to a choice of units, and reflects the \textbf{absence of a mass/length scale in the model}.

Choptuik studies one-parameter families of solutions $\mathcal{S}[p]$. The parameter $p$ characterizes the strength of the gravitational self-interaction of the scalar field. These solutions are obtained by evolving initially in-going packets (shells) of scalar field.\\
For each family there is a value $p_{weak}$ such that in the limit $p\xrightarrow{}p_{weak}$ you recover flat spacetime and the scalar field evolution is simply a solution of the linear wave equation: the scalar wavepacket implodes through $r=0$ and then escapes to infinity (\textcolor{red}{?}).\\
At the other extreme, there is a value $p_{strong}$ such that in the limit $p\xrightarrow{}p_{strong}$ you end up forming a black hole in the collapse of the packet, and an arbitrarily small fraction of the scalar field escapes to infinity (\textcolor{red}{does it mean that we would need to wait an infinite time to see that fraction at infinity? Or is it just the asymptotic behaviour, so that in the exact $p_{strong}$ case you would see nothing at infinity?}).\\
In between there is, geometrically, a \textbf{critical parameter} value $p^*$ where black hole formation first occurs. We can assume $p_{weak}<p^*<p_{strong}$ and refer to solutions as subcritical and supercritical according to whether we are below or above $p^*$. The quantity $|p-p^*|$ is, in both regimes, a natural choice to discuss the phenomenology of the solutions.

In the strong-field, near-critical dynamics $p\xrightarrow{}p^*$ Choptuik conjectures that:\\
(1) the precisely critical behaviour is universal (independent of the particular initial profile chosen for the field);\\
(2) in terms of certain variables, the field profiles of the critical evolution at frozen time will be the same as one rescales the variables by some universal constant $\Delta$. In other words, if one looks at the profiles at a certain geometric time $T$ and then at a later time on scales $e^{\Delta}$ smaller, then the same profiles will appear; then one waits for an additional interval $\delta T$ and zooms in by an additional factor $e^{\Delta}$, again the same profiles.\\
This only happens for strong-field dynamics, that is we are close to $r=0$.

\textbf{A precisely critical configuration will be characterized by an infinite series of echoes in the field profiles, as well as in any other form-invariant quantity} such as $a$, $m/r$, $dm/dr$... which arise from dynamics unfolding on increasingly smaller spatiotemporal scales. There is a geometric relation between the scales of successive echoes: the sequence will conclude at some \textbf{finite} central proper time $T^*$.

One can study the critical behavior starting from subcritical solutions or also from supercritical. In the latter case, \textbf{empirically, the black hole mass is well described by a powerlaw}
\begin{equation}
    M_{BH}\approx c_f |p-p^*|^{\gamma}
\end{equation}
where $c_f$ is a constant that depends on the family, but $\gamma$ is apparently universal and has a numerical value $\gamma\approx 0.37$.



\section{Universal Scaling and Echoing in Gravitational Collapse of a
Complex Scalar Field\\E. W. Hirschmann and D. M. Eardley}

\textbf{Gravitational collapse has two kinds of possible endstates}. The ﬁrst endstate consists of a \textbf{black hole}, plus some outgoing matter and outgoing gravitational radiation. The second endstate consists of a \textbf{stationary remnant star}, plus some outgoing matter and outgoing gravitational radiation, but no black hole. Choice between these endstates \textbf{depends on initial conditions}; gravitational collapse ends in a black hole only if the gravitational ﬁeld becomes strong enough, in the sense of the singularity theorems. A third possibility, the \textbf{naked} singularity, is thought not to occur due to the cosmic censorship conjecture.

The thought experiment employed by Choptuik, in the context of numerical relativity, is to \textbf{tune across the critical threshold in the space of initial conditions} and study the behavior of quantities at this threshold. The parameter $p$ he chose describes the stregth of gravity in the initial state. He finds evidence that the threshold behavior is somehow universal...

For gravitational collapse of \textbf{fermionic matter} from suitably regular initial conditions, the Chandrasekhar mass sets the scale of minimum mass for any black hole, as long as the initial conditions are suﬃciently regular (meaning we don't use focused beams of ultrarelativistic fermions or something like that). In this case, the black hole mass $M_{BH}(p)$ for fermionic configurations  behaves in a simple and rather uninteresting way at threshold: \textbf{it is a step function of} $p$.

For gravitational collapse of \textbf{bosonic matter} from regular initial conditions, we do not find a step function! In spherically symmetric collapse of a massless real scalar ﬁeld $\phi$ coupled to gravity, Choptuik ﬁnds a \textbf{power-law behavior}
\begin{equation}
    M_{BH}(p) \approx (p-p^*)^{\gamma} \qquad \gamma \approx 0.37
\end{equation}
and conjectures that $\gamma$ may be universal.


 For a massless scalar ﬁeld with no self-coupling, no bound star can exist (\textcolor{red}{is that because there is nothing that may play the role of pressure?} so that we either collapse due to gravity or blow away at infinity?), so that the endstate consists of outgoing scalar radiation, plus a possible black hole.
 
 Furthermore, exactly at the threshold
  $ p^* $
 
 , he ﬁnds a unique ﬁeld conﬁguration acting as an attractor for all nearby initial conditions. This ﬁeld conﬁguration, which we will call a \textbf{choptuon}, has a \textbf{discrete self-similarity}, by virtue of which it exhibits a striking, recurrent \textbf{echoing behavior: it repeats itself at ever-decreasing time- and length-scales}.
 \begin{align}
     &\phi(t^{\prime},r^{\prime})=\phi(t,r)\\
     &t^{\prime}=e^{-n\Delta}t \qquad r^{\prime}=e^{-n\Delta}r \qquad ds^{\prime 2}=e^{-2n\Delta}ds^2 \qquad n=1,2,3,...
 \end{align}
 with $(t,r)$ spherical coordinates and $\Delta$ a constant to be determined numerically. The solution is thus \textbf{invariant under a discrete family of scale transformations}.
 
 \textcolor{red}{Choptuons amount to a new kind of counterexample to some formulations of the cosmic censorship conjecture}, a counterexample that cannot be blamed on bad choice of matter ﬁelds. Technically they are a counterexample because regions of arbitrarily strong curvature are visible to observers at future null inﬁnity.\\
 Even more importantly, choptuons represent in principle a means by which eﬀects of extremely strong ﬁeld gravity, even quantum gravity, can be observable in the present universe.
 
 If we use a \textbf{complex scalar field} rather than a real one, echoing is allowed to occur in the form of \textbf{phase oscillations}: $\phi$ changes phase but not amplitude under a scale transformation. In other words, we can interpret the rescaling as acting on the amplitude, or on the phase, or both.
 \begin{align}
     &\phi(t,r)=(-t)^{i\omega}f(-r/t)\\
     &t^{\prime}=e^{-\lambda}t \qquad r^{\prime}=e^{-\lambda}r \qquad \phi(t^{\prime},r^{\prime})=e^{-i\omega\lambda}\phi(t,r) \qquad 0<\lambda<\infty
 \end{align}
 This field is continuously self-similar. It exhibits \textbf{linear phase oscillations, a form of the echoing, superimposed on exact continuous scale symmetry}.



\section{More On Critical Collapse of Axion-Dilaton System in Dimension Four
\\L. \'Alvarez-Gaumé and Ehsan Hatefi}
